Fixed Points and Noetherian Topologies

This paper provides a canonical construction of a Noetherian least fixed point topology. While such least fixed point are not Noetherian in general, we prove that under a mild assumption, one can use a topological minimal bad sequence argument to prove that they are. We then apply this fixed point theorem to rebuild known Noetherian topologies with a uniform proof. In the case of spaces that are defined inductively (such as finite words and finite trees), we provide a uniform definition of a divisibility topology using our fixed point theorem. We then prove that the divisibility topology is a generalisation of the divisibility preorder introduced by Hasegawa in the case of well-quasi-orders.

==> globals/boxes.tex <==
% ALERT PANEL
 \newlength{\alertmessagelength}%
 \newcommand*\alertmessagepanel[3]{%
  \begin{center} %
  \noindent % No indentation
  \begin{tikzpicture} %
  \node[draw=#1!80, rounded corners=5pt, inner sep=11pt]{ % Add a little bit of transparency
  $\begin{array}{l} % One-cell table
  \includegraphics{{#2}} % Alert icon
  \end{array}$ %
  \begin{minipage}{0.7\linewidth}
  \footnotesize #3
  \end{minipage} % Box which handles paragraphs, limited to 10cm
  }; %
  \end{tikzpicture} %
  \end{center} %
  \par % Get back the indentation
 }%

 % ERROR ALERT
 \newcommand*\alerterror[1]{%
  \alertmessagepanel{myRed}{images/alertmessage-error.png}{#1}%
 }%

 % ERROR WARNING
 \newcommand*\alertwarning[1]{%
  \alertmessagepanel{myOrange}{images/alertmessage-warning.png}{#1}%
 }%

 % ERROR SUCCESS
 \newcommand*\alertsuccess[1]{%
  \alertmessagepanel{myGreen}{images/alertmessage-success.png}{#1}%
 }%

 % ERROR INFO
 \newcommand*\alertinfo[1]{%
  \alertmessagepanel{myDarkBlue}{images/alertmessage-info.png}{#1}%
 }%

 % ERROR QUESTION
 \newcommand*\alertquestion[1]{%
  \alertmessagepanel{myYellow}{images/alertmessage-question.png}{#1}%
 }%

 % ERROR QUESTION
 \newcommand*\alertmore[1]{%
  \alertmessagepanel{myPurple}{images/alertmessage-more.png}{#1}%
 }%

 % ERROR QUESTION
 \newcommand*\alertwip[1]{%
  \alertmessagepanel{myBlack}{images/alertmessage-wip.png}{#1}%
 }%


==> parties/intro_lncs.tex <==
\subparagraph*{Program termination.}

We often use program termination.

\subparagraph*{Well-quasi-orderings.}

\begin{table}
	\centering
	\begin{tabular}{cccc}
		\toprule
		\textbf{Operation} & \textbf{Set}   & \textbf{Order}   & \textbf{WQO} \\
		\midrule
		$\W_1 + \W_2$      & disjoint union & $a \leq b$ iff ? & yes
		\\
		\bottomrule
	\end{tabular}
\end{table}

\subparagraph*{Noetherian spaces.}
\begin{table}
	\centering
	\begin{tabular}{cccc}
		\toprule
		\textbf{Operation} & \textbf{Set}   & \textbf{Order}   &
		\textbf{Noetherian}                                          \\
		\midrule
		$\W_1 + \W_2$      & disjoint union & $a \leq b$ iff ? & yes
		\\
		\bottomrule
	\end{tabular}
\end{table}



